Black-Box Visual Prompt Engineering for Mitigating Object Hallucination in Large Vision Language Models

Large Vision Language Models (LVLMs) often suffer from object hallucination, which undermines their reliability. Surprisingly, we find that simple object-based visual prompting -- overlaying visual cues (e.g., bounding box, circle) on images -- can significantly mitigate such hallucination; however, different visual prompts (VPs) vary in effectiveness. To address this, we propose Black-Box Visual Prompt Engineering (BBVPE), a framework to identify optimal VPs that enhance LVLM responses without needing access to model internals. Our approach employs a pool of candidate VPs and trains a router model to dynamically select the most effective VP for a given input image. This black-box approach is model-agnostic, making it applicable to both open-source and proprietary LVLMs. Evaluations on benchmarks such as POPE and CHAIR demonstrate that BBVPE effectively reduces object hallucination.

==> etc/01_algorithm.tex <==
\begin{algorithm}[t!]
\caption{Visual Prompt Router}
\footnotesize
\begin{algorithmic}[1]
\State \textbf{Input:} $v, t$ \Comment{{\scriptsize $v$: visual prompt, $t$: text prompt}}
\State \textbf{LVLM:} $\mathcal{M}$
\State \textbf{Diffusion Model:} $\mathcal{D}$
\State \textbf{Scoring Model:} $\mathcal{S}$
\State \textbf{Exiting Threshold:} $\mu$

\State $r \leftarrow \mathcal{M}(v, t)$ \Comment{{\scriptsize Get initial response from LVLM}}
\State $s_{\text{cur}} \leftarrow \mathcal{S}(r)$ \Comment{{\scriptsize Score the response}}
\State $f \leftarrow \mathcal{M}(\text{instruction}([v, t, s_{\text{cur}}])$ \Comment{{\scriptsize Get textual feedback from LVLM}}
\State $s_{\text{prev}} \leftarrow s_{\text{cur}}$
\State $gain \leftarrow \infty$

\While{$gain > \mu$}
    \State $v^* \leftarrow \mathcal{D}(v; f)$ \Comment{{\scriptsize Refine $v$ using text-conditional diffusion model}}
    \State $r \leftarrow \mathcal{M}(v^*, t)$ \Comment{{\scriptsize Get response from LVLM}}
    \State $s_{\text{cur}} \leftarrow \mathcal{S}(r)$ \Comment{{\scriptsize Score the response}}
    \State $f \leftarrow \mathcal{M}(\text{instruction}([v^*, t, s_{\text{cur}}]))$ \Comment{{\scriptsize Get textual feedback from LVLM}}
    \State $gain \leftarrow s_{\text{cur}} - s_{\text{prev}}$
    \State $s_{\text{prev}} \leftarrow s_{\text{cur}}$
    \State $v \leftarrow v^*$
\EndWhile

\Return $v^*$, $r$ \Comment{{\scriptsize Return refined visual prompt and response}}
\end{algorithmic}
\end{algorithm}

==> figures/02_motivation.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{figures/motivation.png}
    \vspace{-5mm}
    \caption{
        \textbf{Oracle visual prompting can achieve near-perfect score in object hallucination benchmarks~\cite{li2023evaluating,rohrbach2018object}.}
        % Second question arises here.
        Different VPs elicit varied responses, but not all are equally effective; their success depends on the specific characteristics of the image.
        To eliminate randomness and accurately assess the impact of visual prompting, all responses are generated using greedy decoding.
        While most VPs yield comparable results, an oracle -- where an optimal VP is applied per image -- can lead to significant performance improvements.
        Now question arises: \textbf{(Q2)} Can we systematically learn the optimal VPs?
        % \todo{emphasize -- move fig 1}
    }
    % \kz{should we show the images with visual prompts applied, maybe more intuitive}}% \sm{included in figure 1}
    \vspace{-2mm}
    \label{fig:motivation}
\end{figure*}

==> figures/04_attention.tex <==
\begin{figure}[t!]
    \centering
    % \vspace{-2mm}
    \includegraphics[width=\linewidth]{figures/attention.png}
    \vspace{-5mm}
    \caption{
        \textbf{Effect of visual prompting on attention and answer correction in LLaVA 1-5.}
        % \kz{are we the first one observing this phenomenon and illustrating?} \sm{Previous works focus on the relationship between visual prompting and visual grounding. AFAIK, we are the first to use visual prompting for object hallucination and to explain those phenomenon by attention.}
    }%
    \vspace{-3mm}
    \label{fig:attention}
\end{figure}

==> tables/01_01_pope_open.tex <==
\begin{table*}[t!]
    \centering
    \small
    \setlength{\tabcolsep}{5pt} % base value: 6pt
    \scalebox{1}{
    \begin{tabular}{y{40}y{46}x{30}x{30}x{30}x{30}x{30}x{30}x{30}x{30}}
    \toprule
    \multirow{2}{*}{\textbf{Setup}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{LLaVA 1.5~\cite{liu2023visual}}} & \multicolumn{4}{c}{\textbf{InstructBLIP~\cite{dai2024instructblip}}} \\
    \arrayrulecolor{gray} \cmidrule(lr){3-6} \cmidrule(lr){7-10}
     &  & Acc. & Prec. & Rec. & F1 & Acc. & Prec. & Rec. & F1 \\
    \midrule
    \multirow{6}{*}{Random} 
     & \textit{base} & 89.60 & 88.77 & 90.67 & 89.71 & 90.23 & 92.95 & 87.07 & 89.91 \\
     & \textit{random} & 89.46 & 89.07 & 89.95 & 89.51 & 89.75 & 91.76 & 87.35 & 89.50 \\
     & \textit{best singular} & 90.40 & 90.67 & 90.07 & 90.37 & 89.97 & 91.89 & 87.67 & 89.73 \\
     & \textit{routing} & - & - & - & - & - & - & - & - \\
    \arrayrulecolor{gray!50}\cmidrule(lr){2-10}
     & Oracle (V) & 94.33 & - & - & - & - & - & - & - \\
     % & Oracle (VQ) & - & - & - & - & - & - & - & - \\
    \midrule
    \multirow{6}{*}{Popular} 
     & \textit{base} & 86.20 & 83.23 & 90.67 & 86.79 & 83.43 & 81.17 & 87.07 & 84.01 \\
     & \textit{random} & 86.20 & 83.68 & 89.96 & 86.70 & 83.12 & 80.54 & 87.35 & 83.80 \\
     & \textit{best singular} & 86.70 & 84.38 & 90.07 & 87.13 & 84.13 & 81.88 & 87.67 & 84.67 \\
     & \textit{routing} & - & - & - & - & - & - & - & - \\
    \arrayrulecolor{gray!50}\cmidrule(lr){2-10}
     & Oracle (V) & 91.97 & - & - & - & - & - & - & - \\
     % & Oracle (VQ) & - & - & - & - & - & - & - & - \\
    \midrule
    \multirow{6}{*}{Adversarial} 
     & \textit{base} & 79.73 & 74.40 & 90.67 & 81.73 & 80.73 & 77.28 & 87.07 & 81.88 \\
     & \textit{random} & 79.56 & 74.48 & 89.95 & 81.49 & 79.87 & 75.99 & 87.35 & 81.27 \\
     & \textit{best singular} & 80.30 & 75.35 & 90.07 & 82.05 & 80.20 & 76.28 & 87.67 & 81.58 \\
     & \textit{routing} & - & - & - & - & - & - & - & - \\
    \arrayrulecolor{gray!50}\cmidrule(lr){2-10}
     & Oracle (V) & 86.67 & - & - & - & - & - & - & - \\
     % & Oracle (VQ) & - & - & - & - & - & - & - & - \\
     \bottomrule
    \end{tabular}
    }
    \vspace{\abovetabcapmargin}
    \caption{
        \textbf{Open-source VLAs' results on POPE~\cite{li2023evaluating} benchmark.}
        consistently outperforms
        best singular is reverse blur
        \todo{+baseline}
        \todo{Oracle VQ pick just one}
    }
    \vspace{\belowtabcapmargin}
    \label{tab:pope_open}
\end{table*}

==> tables/01_02_pope_closed.tex <==
\begin{table*}[t!]
    \centering
    \small
    \setlength{\tabcolsep}{5pt} % base value: 6pt
    \scalebox{1}{
    \begin{tabular}{y{40}y{46}x{30}x{30}x{30}x{30}x{30}x{30}x{30}x{30}}
    \toprule
    \multirow{2}{*}{\textbf{Setup}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{GPT-4o~\cite{openai2024gpt4o}}} & \multicolumn{4}{c}{\textbf{Claude-3.0-Sonnet~\cite{anthropic2024claude}}} \\
    \arrayrulecolor{gray} \cmidrule(lr){3-6} \cmidrule(lr){7-10}
     &  & Acc. & Prec. & Rec. & F1 & Acc. & Prec. & Rec. & F1 \\
    \midrule
    \multirow{6}{*}{Random} 
     & \textit{base} & - & - & - & - & 79.93 & 98.18 & 61.00 & 75.25 \\
     & \textit{random} & - & - & - & - & 78.91 & 97.74 & 59.18 & 73.71 \\
     & \textit{best singular} & - & - & - & - & 80.10 & 97.78 & 61.60 & 75.58 \\
     & \textit{routing} & - & - & - & - & - & - & - & - \\
    \arrayrulecolor{gray!50}\cmidrule(lr){2-10}
     & Oracle (V) & - & - & - & - & 85.87 & - & - & - \\
     & Oracle (VQ) & - & - & - & - & - & - & - & - \\
    \midrule
    \multirow{6}{*}{Popular} 
     & \textit{base} & - & - & - & - & 78.43 & 93.56 & 61.07 & 73.90 \\
     & \textit{random} & - & - & - & - & 77.48 & 93.24 & 59.24 & 72.44 \\
     & \textit{best singular} & - & - & - & - & 78.70 & 93.90 & 61.60 & 74.40 \\
     & \textit{routing} & - & - & - & - & - & - & - & - \\
    \arrayrulecolor{gray!50}\cmidrule(lr){2-10}
     & Oracle (V) & - & - & - & - & 84.87 & - & - & - \\
     & Oracle (VQ) & - & - & - & - & - & - & - & - \\
    \midrule
    \multirow{6}{*}{Adversarial} 
     & \textit{base} & - & - & - & - & 77.13 & 89.82 & 61.20 & 72.80 \\
     & \textit{random} & - & - & - & - & 75.90 & 88.83 & 59.25 & 71.07 \\
     & \textit{best singular} & - & - & - & - & 76.90 & 88.76 & 61.60 & 72.73 \\
     & \textit{routing} & - & - & - & - & - & - & - & - \\
    \arrayrulecolor{gray!50}\cmidrule(lr){2-10}
     & Oracle (V) & - & - & - & - & 83.53 & - & - & - \\
     & Oracle (VQ) & - & - & - & - & - & - & - & - \\
     \bottomrule
    \end{tabular}
    }
    \vspace{\abovetabcapmargin}
    \caption{
        \textbf{Proprietary VLAs' results on POPE~\cite{li2023evaluating} benchmark.}
        consistently outperforms
        best singular is reverse blur
    }
    \vspace{\belowtabcapmargin}
    \label{tab:pope_closed}
\end{table*}

==> tables/02_01_chair_open.tex <==
\begin{table}[t!]
    \begin{center}
    \begin{small}
    \setlength{\tabcolsep}{4pt} % base value: 6pt
    \scalebox{0.9}{
    \begin{tabular}{lx{37}x{37}x{37}x{37}}
        \toprule
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{LLaVA 1.5}} & \multicolumn{2}{c}{\textbf{InstructBLIP}} \\
        \arrayrulecolor{gray} \cmidrule(lr){2-3} \cmidrule(lr){4-5}
         & CHAIR$_S$ & CHAIR$_I$ & CHAIR$_S$ & CHAIR$_I$ \\
        \midrule
        \textit{base} & - & - & - & - \\
        \textit{random} & - & - & - & - \\
        \textit{best singular} & - & - & - & - \\
        \textit{routing} & - & - & - & - \\
        \arrayrulecolor{gray!50}\cmidrule(lr){1-5}
        Oracle & - & - & - & - \\
        \arrayrulecolor{gray} \midrule
        \textit{base} & - & - & - & - \\
        \textit{random} & - & - & - & - \\
        \textit{best singular} & - & - & - & - \\
        \textit{routing} & - & - & - & - \\
        \arrayrulecolor{gray!50}\cmidrule(lr){1-5}
        Oracle & - & - & - & - \\
        \bottomrule
    \end{tabular}
    }
    \end{small}
    \end{center}
    \vspace{\abovetabcapmargin}
    \captionof{table}{
        \textbf{Open-source VLA's results on CHAIR~\cite{rohrbach2018object} benchmark.}
        Ours significantly reduces object hallucinations in description generation
    }
    \vspace{\belowtabcapmargin}
    \label{tab:chair_open}
\end{table}

==> tables/02_02_chair_closed.tex <==
\begin{table}[t!]
    \begin{center}
    \begin{small}
    \setlength{\tabcolsep}{4pt} % base value: 6pt
    \scalebox{0.9}{
    \begin{tabular}{lx{37}x{37}x{37}x{37}}
        \toprule
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{GPT-4o}} & \multicolumn{2}{c}{\textbf{Claude-3.0-Sonnet}} \\
        \arrayrulecolor{gray} \cmidrule(lr){2-3} \cmidrule(lr){4-5}
         & CHAIR$_S$ & CHAIR$_I$ & CHAIR$_S$ & CHAIR$_I$ \\
        \midrule
        \textit{base} & - & - & - & - \\
        \textit{random} & - & - & - & - \\
        \textit{best singular} & - & - & - & - \\
        \textit{routing} & - & - & - & - \\
        \arrayrulecolor{gray!50}\cmidrule(lr){1-5}
        Oracle & - & - & - & - \\
        \arrayrulecolor{gray} \midrule
        \textit{base} & - & - & - & - \\
        \textit{random} & - & - & - & - \\
        \textit{best singular} & - & - & - & - \\
        \textit{routing} & - & - & - & - \\
        \arrayrulecolor{gray!50}\cmidrule(lr){1-5}
        Oracle & - & - & - & - \\
        \bottomrule
    \end{tabular}
    }
    \end{small}
    \end{center}
    \vspace{\abovetabcapmargin}
    \captionof{table}{
        \textbf{Proprietary VLA's results on CHAIR~\cite{rohrbach2018object} benchmark.}
        Ours significantly reduces object hallucinations in description generation
    }
    \vspace{\belowtabcapmargin}
    \label{tab:chair_closed}
\end{table}

==> tables/02_03_gpt4o.tex <==
\begin{table}[t!]
    \begin{center}
    \begin{small}
    \setlength{\tabcolsep}{1pt} % base value: 6pt
    \scalebox{0.8}{
    \begin{tabular}{lx{35}x{35}x{35}x{35}x{35}x{35}}
        \toprule
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{6}{c}{\textbf{LLaVA 1.5}} \\
        \arrayrulecolor{gray} \cmidrule(lr){2-7}
         & Accuracy & Detail & Compreh. & Relev. & Robust & Total{\up} \\
        \midrule
        \textit{base} & $7.08$ & $6.63$ & $6.67$ & $7.35$ & $7.51$ & $35.24$ \\
        \textit{random} & $6.38$ & $6.21$ & $6.25$ & $6.85$ & $6.84$ & $32.52$ \\
        \textit{best singular$^{\dagger}$} & $6.53$ & $6.30$ & $6.34$ & $6.92$ & $6.92$ & $33.00$ \\
        \textbf{BBVPE} & 7.24 & 6.86 & 6.95 & 7.63 & 7.70 & $36.38$ \\
        \arrayrulecolor{gray!50}\cmidrule(lr){1-7}
        Oracle & 7.59 & 7.27 & 7.30 & 8.03 & 8.10 & $38.29$ \\
        \bottomrule
    \end{tabular}
    }
    \end{small}
    \end{center}
    \vspace{\abovetabcapmargin}
    \captionof{table}{
        \textbf{GPT-4o evaluation on image descriptions generated by LLaVA.}
        ${\dagger}$ Best singular visual prompt is `center point'.
    }
    \vspace{\belowtabcapmargin}
    \label{tab:gpt_evaluation}
\end{table}

% \begin{table}[t!]
%     \begin{center}
%     \begin{small}
%     \setlength{\tabcolsep}{1pt} % base value: 6pt
%     \scalebox{0.8}{
%     \begin{tabular}{lx{35}x{35}x{35}x{35}x{35}x{35}}
%         \toprule
%         \multirow{2}{*}{\textbf{Method}} & \multicolumn{6}{c}{\textbf{LLaVA 1.5~\cite{liu2023improved}}} \\
%         \arrayrulecolor{gray} \cmidrule(lr){2-7}
%          & Accuracy & Detail & Compreh. & Relev. & Robustness & Total \\
%         \midrule
%         \textit{base} & $7.08_{(\pm 1.70)}$ & $6.63_{(\pm 1.37)}$ & $6.67_{(\pm 1.43)}$ & $7.35_{(\pm 1.41)}$ & $7.51_{(\pm 1.76)}$ & $35.24_{(\pm 7.16)}$ \\
%         \textit{random} & $6.38_{(\pm 1.85)}$ & $6.21_{(\pm 1.47)}$ & $6.25_{(\pm 1.50)}$ & $6.85_{(\pm 1.38)}$ & $6.84_{(\pm 1.95)}$ & $32.52_{(\pm )}$ \\
%         \textit{best singular} & $6.53_{(\pm 1.76)}$ & $6.30_{(\pm 1.39)}$ & $6.34_{(\pm 1.42)}$ & $6.92_{(\pm 1.45)}$ & $6.92_{(\pm 1.87)}$ & $33.00_{(\pm 7.32)}$ \\
%         \textit{BBVPE} & - & - & - & - & - & $36.38_{(\pm )}$ \\
%         \arrayrulecolor{gray!50}\cmidrule(lr){1-7}
%         Oracle & - & - & - & - & - & $38.29_{(\pm )}$ \\
%         \bottomrule
%     \end{tabular}
%     }
%     \end{small}
%     \end{center}
%     \vspace{\abovetabcapmargin}
%     \captionof{table}{
%         \textbf{GPT-4o.}
%         arrow arrow
%     }
%     \vspace{\belowtabcapmargin}
%     \label{tab:gpt_evaluation}
% \end{table}
